Null-stream veto for two co-located detectors: Implementation issues

Time-series data from multiple gravitational wave (GW) detectors can be linearly combined to form a null-stream, in which all GW information will be cancelled out. This null-stream can be used to distinguish between actual GW triggers and spurious noise transients in a search for GW bursts using a network of detectors. The biggest source of error in the null-stream analysis comes from the fact that the detector data are not perfectly calibrated. In this paper, we present an implementation of the null-stream veto in the simplest network of two co-located detectors. The detectors are assumed to have calibration uncertainties and correlated noise components. We estimate the effect of calibration uncertainties in the null-stream veto analysis and propose a new formulation to overcome this. This new formulation is demonstrated by doing software injections in Gaussian noise.

==> Makefile <==
# Makefile for LaTeX documents

SHELL       =  /bin/sh

TEX_FILES   =  $(wildcard $(CURDIR)/*.tex)
STY_FILES   =  $(wildcard $(CURDIR)/*.sty)
CLS_FILES   =  $(wildcard $(CURDIR)/*.cls)
BIB_FILES   =  $(wildcard $(CURDIR)/*.bib)

MAIN_FILE   =  $(wildcard $(CURDIR)/ColocNS.tex)
ifneq ($(MAIN_FILE),)
  TEX_FILE  = $(MAIN_FILE)
else
  TEX_FILE  = $(TEX_FILES)
endif
ifneq ($(words $(TEX_FILE)), 1)
  $(error Error: There is more than one .tex file in the current directory)
endif


BASE_FILE   =  $(basename $(TEX_FILE))
DVI_FILE    =  $(addsuffix .dvi, $(BASE_FILE))
PDF_FILE    =  $(addsuffix .pdf, $(BASE_FILE))
PS_FILE     =  $(addsuffix .ps, $(BASE_FILE))
PS2UP_FILE  =  $(addsuffix _2up.ps, $(BASE_FILE))

BIBTEX      =  $(if $(shell grep '\\bibliography{' $(TEX_FILES)), bibtex, :)

FIG_FIGURES =  $(sort $(wildcard $(CURDIR)/figures/*.fig))
EPS_FROMFIG =  $(addsuffix .eps, $(basename $(FIG_FIGURES)))
EPS_FIGURES =  $(sort $(wildcard $(CURDIR)/figures/*.eps) $(EPS_FROMFIG))
PDF_FIGURES =  $(addsuffix .pdf, $(basename $(EPS_FIGURES)))

.DELETE_ON_ERROR:

.PHONY:         all dvi ps ps2up pdf clean publish

all:            dvi ps ps2up pdf

dvi:            $(DVI_FILE)

ps:             $(PS_FILE)

ps2up:          $(PS2UP_FILE)

pdf:            $(PDF_FILE)

clean:
	     	-rm -f *~ >/dev/null 2>&1
	     	-rm -f *.aux >/dev/null 2>&1
	     	-rm -f *.lof >/dev/null 2>&1
	     	-rm -f *.lot >/dev/null 2>&1
	     	-rm -f *.toc >/dev/null 2>&1
	     	-rm -f *.log >/dev/null 2>&1
	     	-rm -f *.bbl >/dev/null 2>&1
	     	-rm -f *.blg >/dev/null 2>&1
	     	-rm -f *.brf >/dev/null 2>&1
	     	-rm -f *.end >/dev/null 2>&1
	     	-rm -f *.out >/dev/null 2>&1
	     	-rm -f *.dvi >/dev/null 2>&1
	     	-rm -f *.ps >/dev/null 2>&1
	     	-rm -f *.tpt >/dev/null 2>&1
	     	-rm -f *.pdf >/dev/null 2>&1
	     	-rm -f *.bak >/dev/null 2>&1
	     	-rm -f $(EPS_FROMFIG) >/dev/null 2>&1
	     	-rm -f figures/*.pdf >/dev/null 2>&1

$(DVI_FILE): 	$(TEX_FILES) $(CLS_FILES) $(STY_FILES) $(BIB_FILES) $(EPS_FIGURES)
	     	latex $(TEX_FILE)
	     	$(BIBTEX) $(BASE_FILE)
	     	latex $(TEX_FILE)
	     	latex $(TEX_FILE)
	     	latex $(TEX_FILE)

$(PS_FILE):     $(DVI_FILE) $(EPS_FIGURES)
	        dvips -o $(PS_FILE) $(DVI_FILE)

$(PS2UP_FILE):  $(PS_FILE)
	        psnup -2 $(PS_FILE) $(PS2UP_FILE)

$(PDF_FILE):    $(TEX_FILES) $(PDF_FIGURES)
	        pdflatex $(TEX_FILE)
	        $(BIBTEX) $(BASE_FILE)
	        pdflatex $(TEX_FILE)
	        pdflatex $(TEX_FILE)
	        pdflatex $(TEX_FILE)

publish:	$(PS_FILE) $(PS2UP_FILE) $(PDF_FILE)
	        rsync --rsh=ssh -avz $(PS_FILE) $(USER)@sshserv.aei.mpg.de:/
	        rsync --rsh=ssh -avz $(PS2UP_FILE) $(USER)@sshserv.aei.mpg.de:/
	        rsync --rsh=ssh -avz $(PDF_FILE) $(USER)@sshserv.aei.mpg.de:/

.SUFFIXES:
.SUFFIXES:   .fig .eps .pdf

%.eps:       %.fig
	     fig2dev -L eps $< $@

%.pdf:       %.eps
	     epstopdf $<

